An Empirical Investigation of Global and Local Normalization for Recurrent Neural Sequence Models Using a Continuous Relaxation to Beam Search

Globally normalized neural sequence models are considered superior to their locally normalized equivalents because they may ameliorate the effects of label bias. However, when considering high-capacity neural parametrizations that condition on the whole input sequence, both model classes are theoretically equivalent in terms of the distributions they are capable of representing. Thus, the practical advantage of global normalization in the context of modern neural methods remains unclear. In this paper, we attempt to shed light on this problem through an empirical study. We extend an approach for search-aware training via a continuous relaxation of beam search (Goyal et al., 2017b) in order to enable training of globally normalized recurrent sequence models through simple backpropagation. We then use this technique to conduct an empirical study of the interaction between global normalization, high-capacity encoders, and search-aware optimization. We observe that in the context of inexact search, globally normalized neural models are still more effective than their locally normalized counterparts. Further, since our training approach is sensitive to warm-starting with pre-trained models, we also propose a novel initialization strategy based on self-normalization for pre-training globally normalized models. We perform analysis of our approach on two tasks: CCG supertagging and Machine Translation, and demonstrate the importance of global normalization under different conditions while using search-aware training.

==> ccg-tab.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{}       & Uni   & Bi & MT    \\ \hline
\multirow{3}{*}{CE} & pre    & 77.76 & 93.29 & 27.62      \\ \cline{2-5} 
                    & local  & 83.9  & 93.76 & 29.28      \\ \cline{2-5} 
                    & global & 83.93 & 93.73 & 26.24     \\ \hline
\multirow{3}{*}{L2} & pre    & 73.83 & 91.94 & 26.63     \\ \cline{2-5} 
                    & local  & 83.35 & 92.78 & 27.71     \\ \cline{2-5} 
                    & global & 85.50 & 92.63 & 29.27     \\ \hline
\end{tabular}
\caption{\label{ccg} {\bf Accuracy results on CCG supertagging} (\emph{Uni}, \emph{Bi}) and {\bf BLEU results on Machine Translation} (\emph{MT}). \emph{Uni} and \emph{Bi} refer to the unidirectional and bidirectional encoders respectively with fixed attention tagging decoder. \emph{CE} refers to training cross-entropy teacher-forcing method. \emph{L2} refers to a training of self-normalized models with L2 regularization on logZ. \emph{pre} refers to the model used for pretraining. \emph{local} and \emph{global} refer to search-aware soft beam optimization for locally normalized and globally normalized models respectively.}
\end{table}

==> mt-tab.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{3}{|l|}{CE} & \multicolumn{3}{l|}{L2} \\ \hline
pre    & local  & global & pre    & local & global \\ \hline
27.62  & 29.30  & 26.24  & 26.63  & 27.71 & 29.23  \\ \hline
\end{tabular}
\caption{\label{mt-old} BLEU results on de-en Machine Translation. \emph{CE} refers to training cross-entropy teacher-forcing method. \emph{L2} refers to a training with L2 regularization on logZ. \emph{pre} refers to the model used for pretraining. \emph{loc} and \emph{glob} refer to search-aware soft beam optimization for locally normalized and globally normalized models respectively.}
\end{table}
